Closed geodesics with prescribed intersection numbers

Let $(\Sigma, g)$ be a closed, oriented, negatively curved surface, and fix pairwise disjoint simple closed geodesics $\gamma_{\star,1}, \dots \gamma_{\star, r}$. We give an asymptotic growth as $L \to +\infty$ of the number of primitive closed geodesic of length less than $L$ intersecting $\gamma_{\star,j}$ exactly $n_j$ times, where $n_1, \dots, n_r$ are fixed nonnegative integers. This is done by introducing a dynamical scattering operator associated to the surface with boundary obtained by cutting $\Sigma$ along $\gamma_{\star,1}, \dots, \gamma_{\star, r}$ and by using the theory of Pollicott-Ruelle resonances for open systems.

==> bib.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Yann Chaubet at 2018-05-23 15:05:03 +0200 


%% Saved with string encoding Unicode (UTF-8) 



@article{faure2008semi,
	Author = {F. Faure and N. Roy and J. Sj{\"o}strand},
	Date-Added = {2018-05-23 13:04:03 +0000},
	Date-Modified = {2018-05-23 13:04:59 +0000},
	Journal = {Open Math. Journal},
	Title = {Semi-classical approach for Anosov diffeomorphisms and Ruelle resonances},
	Year = {2008}}

@book{lerner,
	Author = {N. Lerner},
	Date-Added = {2018-03-29 13:26:47 +0000},
	Date-Modified = {2018-03-29 13:28:39 +0000},
	Title = {A First Course on Pseudo-Differential Operators},
	Year = {2017}}

@unpublished{cinf,
	Author = {M. Asoaka, K. Irie},
	Date-Added = {2016-09-19 14:11:48 +0000},
	Date-Modified = {2016-09-19 16:24:38 +0000},
	Note = {http://arxiv.org/abs/1512.06336v2},
	Title = {A $\mathcal{C}^\infty$ closing lemma for Hamiltonian diffeomorphisms of closed surfaces}}

@article{pac,
	Author = {M. Schwarz},
	Date-Added = {2016-09-19 14:07:39 +0000},
	Date-Modified = {2016-09-19 14:08:35 +0000},
	Journal = {Pacific J. Math.},
	Number = {2},
	Pages = {419-461},
	Title = {On the action spectrum for closed symplectically aspherical manifolds},
	Volume = {193},
	Year = {2000}}

@article{burghelea2006euler,
  title={Euler structures, the variety of representations and the Milnor--Turaev torsion},
  author={Burghelea, Dan and Haller, Stefan},
  journal={Geometry \& Topology},
  volume={10},
  number={2},
  pages={1185--1238},
  year={2006},
  publisher={Mathematical Sciences Publishers}
}

@article{hutchings1999circle,
  title={Circle-valued Morse theory and Reidemeister torsion},
  author={Hutchings, Michael and Lee, Yi-Jen},
  journal={Geometry \& Topology},
  volume={3},
  number={1},
  pages={369--396},
  year={1999},
  publisher={Mathematical Sciences Publishers}
}

@article{turaev1990euler,
  title={Euler structures, nonsingular vector fields, and torsions of Reidemeister type},
  author={Turaev, Vladimir Georgievich},
  journal={Mathematics of the USSR-Izvestiya},
  volume={34},
  number={3},
  pages={627},
  year={1990},
  publisher={IOP Publishing}
}

@article{dang2017spectral,
  title={Spectral analysis of Morse-Smale flows II: resonances and resonant states},
  author={Dang, Nguyen Viet and Riviere, Gabriel},
  journal={arXiv preprint arXiv:1703.08038},
  year={2017}
}

@book{simon2005trace,
  title={Trace ideals and their applications},
  author={Simon, Barry},
  number={120},
  year={2005},
  publisher={American Mathematical Soc.}
}

@book{kosinski,
  title={Differential manifolds},
  author={Kosinski, Antoni A},
  year={2013},
  publisher={Courier Corporation}
}
@article{brouder2015continuity,
  title={Continuity of the fundamental operations on distributions having a specified wave front set (with a counter example by Semyon Alesker)},
  author={Brouder, Christian and Dang, Nguyen Viet and H{\'e}lein, Fr{\'e}d{\'e}ric},
  journal={Studia Mathematica},
  volume={232},
  number={3},
  pages={201--226},
  year={2015}
}

@phdthesis{he2010odd,
  title={Odd dimensional symplectic manifolds by Zhenqi He.},
  author={He, Zhenqi},
  year={2010},
  school={Massachusetts Institute of Technology}
}

@article{yan1996hodge,
  title={Hodge structure on symplectic manifolds},
  author={Yan, Dong},
  journal={advances in mathematics},
  volume={120},
  number={1},
  pages={143--154},
  year={1996},
  publisher={Academic Press}
}

@article{mathieu1995harmonic,
  title={Harmonic cohomology classes of symplectic manifolds},
  author={Mathieu, Olivier},
  journal={Commentarii Mathematici Helvetici},
  volume={70},
  number={1},
  pages={1--9},
  year={1995},
  publisher={Springer}
}

@article{libermann,
  title={Symplectic Geometry and Analytical Mechanics (D. Reidel Publishing Company, Dordrecht)},
  author={Libermann, P and Marle, CM},
  year={1987}
}

@article{guillemin2001symplectic,
  title={Symplectic Hodge theory and the d$\delta$-lemma},
  author={Guillemin, V},
  journal={preprint, Massachusetts Institute of Technology},
  year={2001}
}
@article{brylinski1988differential,
  title={A differential complex for Poisson manifolds},
  author={Brylinski, Jean-Luc},
  journal={Journal of differential geometry},
  volume={28},
  number={1},
  pages={93--114},
  year={1988},
  publisher={Lehigh University}
}


@article{harvey1979fundamental,
  title={Fundamental solutions in complex analysis Part I. The Cauchy Riemann operator},
  author={Harvey, Reese and Polking, John and others},
  journal={Duke Mathematical Journal},
  volume={46},
  number={2},
  pages={253--300},
  year={1979},
  publisher={Duke University Press}
}


@article{dang2015equidistribution,
  title={Equidistribution of the conormal cycle of random nodal sets},
  author={Dang, Nguyen Viet and Rivi{\`e}re, Gabriel},
  journal={arXiv preprint arXiv:1509.00228},
  year={2015}
}
@article{zworski2018commentary,
  title={Commentary on ‚ÄúDifferentiable dynamical systems‚Äù by Stephen Smale},
  author={Zworski, Maciej},
  journal={Bulletin of the American Mathematical Society},
  volume={55},
  number={3},
  pages={331--336},
  year={2018}
}


@article{Rumin,
  title={Analytic torsions on contact manifolds},
  author={Rumin, Michel and Seshadri, Neil},
  booktitle={Annales de l'Institut Fourier},
  volume={62},
  number={2},
  pages={727--782},
  year={2012}
}


@article{friedl20143,
  title={3-manifolds that can be made acyclic},
  author={Friedl, Stefan and Nagel, Matthias},
  journal={arXiv preprint arXiv:1412.4280},
  year={2014}
}


@book{botttu,
  title={Differential forms in algebraic topology},
  author={Bott, Raoul and Tu, Loring W},
  volume={82},
  year={2013},
  publisher={Springer Science \& Business Media}
}


@book{milnormorse,
  title={Morse theory.(AM-51)},
  author={Milnor, John},
  volume={51},
  year={2016},
  publisher={Princeton university press}
}

@article{dubrovin1984modern,
  title={Modern geometry: methods of homology theory. Part 3: Introduction to homology theory.},
  author={Dubrovin, Boris and BA, Novikov and FOMENKO, SP and others},
  year={1984},
  publisher={Springer}
}

@article{laudenbach2010homologie,
  title={Homologie de Morse dans la perspective de l'Homologie de Floer},
  author={Laudenbach, Fran{\c{c}}ois},
  journal={IMHOTEP: African Journal of Pure and Applied Mathematics},
  volume={9},
  number={2},
  year={2010}
}

@article{laudenbach1992thom,
  title={On the Thom-Smale complex},
  author={Laudenbach, Fran{\c{c}}ois},
  journal={Ast{\'e}risque},
  volume={205},
  pages={219--233},
  year={1992}
}

@inproceedings{hutchings2002,
  title={Reidemeister torsion in generalized Morse theory},
  author={Hutchings, Michael},
  booktitle={Forum Math},
  volume={14},
  pages={209--244},
  year={2002}
}


@article{laudenbach2012transversalite,
  title={Transversalit{\'e}, courants et th{\'e}orie de Morse},
  author={Laudenbach, Fran{\c{c}}ois},
  journal={Un cours de topologie diff{\'e}rentielle, {\'E}ditions de l‚Äô{\'E}cole polytechnique, Palaiseau},
  year={2012}
}

@article{burghelea2011space,
  title={On the Space of Trajectories of a Generic Vector Field},
  author={Burghelea, Dan and Friedlander, Leonid and Kappeler, Thomas},
  journal={arXiv preprint arXiv:1101.0778},
  year={2011}
}


@article{qin2010moduli,
  title={On moduli spaces and CW structures arising from Morse theory on Hilbert manifolds},
  author={Qin, Lizhen},
  journal={Journal of Topology and Analysis},
  volume={2},
  number={04},
  pages={469--526},
  year={2010},
  publisher={World Scientific}
}


@article{dangwitten,
  title={Pollicott-Ruelle spectrum and Witten Laplacians},
  author={Dang, Nguyen Viet and Riviere, Gabriel},
  journal={arXiv preprint arXiv:1709.04265},
  year={2017}
}


@book{mec,
	Author = {C. L. Siegel, J. K. Moser},
	Date-Added = {2016-09-19 14:04:37 +0000},
	Date-Modified = {2016-09-19 14:09:20 +0000},
	Publisher = {Springer-Verlag, New York-Heidelberg},
	Title = {Lectures on Celestial Mechanics},
	Year = {1971}}

@article{mos,
	Author = {J. Moser},
	Date-Added = {2016-09-19 09:04:30 +0000},
	Date-Modified = {2016-09-19 09:06:36 +0000},
	Journal = {Comm. Pure Appl. Math.},
	Pages = {673-692},
	Title = {The analytic invariants of an area-preserving mapping near a hyperbolic fixed point.},
	Volume = {9},
	Year = {1956}}

@unpublished{irie2,
	Author = {Masayuki Asoaka, Kei Irie},
	Date-Added = {2016-08-13 17:13:16 +0000},
	Date-Modified = {2016-08-13 17:15:03 +0000},
	Note = {arXiv:1512.06336v2},
	Title = {A $\mathcal{C}^\infty$ closing lemma for hamiltonian diffeomorphisms of closed surfaces}}

@article{irie,
	Author = {Irie, K.},
	Date-Added = {2016-08-13 16:53:06 +0000},
	Date-Modified = {2016-08-13 16:54:11 +0000},
	Journal = {J. Mod. Dyn.},
	Pages = {357-363},
	Title = {Dense existence of periodic Reeb orbits and ECH spectral invariants},
	Volume = {9},
	Year = {2015}}

@article{vin,
	Author = {D. Cristofaro-Gardiner, M. Hutchings, V. G. B. Ramos},
	Date-Added = {2016-08-13 13:47:37 +0000},
	Date-Modified = {2016-08-13 13:48:44 +0000},
	Journal = {Invent. Math.},
	Number = {1},
	Pages = {187-214},
	Title = {The asymptotics of ECH capacities},
	Volume = {199},
	Year = {2015}}

@unpublished{hut3,
	Author = {D. Cristofaro-Gardiner, M. Hutchings},
	Date-Added = {2016-08-13 13:31:52 +0000},
	Date-Modified = {2016-08-13 13:32:53 +0000},
	Note = {arXiv: 1202.4839v4},
	Title = {From one Reeb orbit to two}}

@article{hut2,
	Author = {Michael Hutchings},
	Date-Added = {2016-08-07 14:38:40 +0000},
	Date-Modified = {2016-08-07 14:40:57 +0000},
	Journal = {Journal of Differential Geometry},
	Number = {2},
	Pages = {231-266},
	Title = {Quantitative embedded contact homology},
	Volume = {88},
	Year = {2011}}

@unpublished{hut,
	Author = {Michael Hutchings},
	Date-Added = {2016-08-07 13:59:24 +0000},
	Date-Modified = {2016-08-07 14:02:38 +0000},
	Note = {arXiv : 1303.5789v2},
	Title = {Lectures notes on embedded contact homology}}

@book{kat,
	Author = {Katok, Anatole and Hasselblatt, Boris},
	Date-Added = {2016-03-22 15:55:29 +0000},
	Date-Modified = {2016-03-22 15:56:49 +0000},
	Publisher = {Cambridge University Press},
	Title = {Introduction to the Modern Theory of Dynamical Systems},
	Year = {1997}}

@book{aud,
	Author = {Mich{\`e}le Audin and Mihai Damian},
	Date-Added = {2016-03-10 16:37:21 +0000},
	Date-Modified = {2016-03-10 16:46:30 +0000},
	Publisher = {Springer},
	Title = {Morse Theory and Floer Homology},
	Year = {2014}}

@article{bart,
	Author = {Bartnik, Robert},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Comm. Pure Appl. Math.},
	Pages = {661--693},
	Title = {The mass of an asymptotically flat manifold},
	Volume = {39},
	Year = {1986}}

@article{geroch,
	Author = {Choquet-Bruhat, Yvonne and Geroch, Robert},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Comm. Math. Phys.},
	Pages = {329-335},
	Title = {Global aspects of the Cauchy problem in General Relativity},
	Volume = {14},
	Year = {1969}}

@unpublished{chru,
	Author = {Chrusciel, Piotr T.},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Month = {March-April},
	Title = {Lectures on Energy in General Relativity},
	Year = {2010}}

@article{witt,
	Author = {Witten, Edward},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Communications in Mathematical Physics},
	Title = {A new proof of the positive energy theorem},
	Volume = {80},
	Year = {1981}}

@article{scho,
	Author = {Schoen, Richard and Yau, Shing Tung},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Physical Review Letters},
	Title = {Positivity of the total mass of a general space-time},
	Volume = {43},
	Year = {1979}}

@incollection{arn,
	Author = {Arnowitt, R. L. and Deser, S. and Misner, C. W.},
	Booktitle = {Gravitation: {A}n introduction to current research},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Pages = {227--265},
	Publisher = {Wiley, New York},
	Title = {The dynamics of general relativity},
	Year = {1962}}

@unpublished{jer,
	Author = {J{\'e}r{\'e}mie Szeftel},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Note = {(Cours en ligne)},
	Title = {Introduction {\`a} la relativit{\'e} g{\'e}n{\'e}rale d'un point de vue math{\'e}matique}}

@article{choq,
	Author = {Y. Choquet-Bruhat, A. E. Fisher and J.E. Marsden},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Isolated Gravitating Systems in General Relativity},
	Title = {Maximal Hypersurfaces and Positivity of Mass},
	Year = {1979}}

@article{hub,
	Author = {Bray, Hubert L.},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Journal of Differential Geometry},
	Title = {Proof of the Riemannian Penrose Inequality using the Positive Mass Theorem},
	Volume = {59},
	Year = {2001}}

@book{wald,
	Author = {Robert M. Wald},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Publisher = {University of Chicago Press},
	Title = {General Relativity},
	Year = {1984}}

@book{sch,
	Author = {Schneider},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Publisher = {Cambridge University Press},
	Title = {Convex Bodies : the Brunn-Minkowski Theory},
	Year = {1993}}

@article{lam,
	Author = {Mau-Kwong George Lam},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Journal = {Cornell University},
	Title = {The Graphs Cases of the Riemannian Positive Mass and Penrose Inequalities in All Dimensions},
	Year = {2010}}

@book{lee,
	Author = {John M. Lee},
	Date-Added = {2016-03-10 16:37:14 +0000},
	Date-Modified = {2016-03-10 16:37:14 +0000},
	Publisher = {Springer},
	Title = {Riemannian manifolds : an introduction to curvature},
	Year = {1997}}

@article{dyatlov2013dynamical,
  title={Dynamical zeta functions for Anosov flows via microlocal analysis},
  author={Dyatlov, Semyon and Zworski, Maciej},
  journal={arXiv preprint arXiv:1306.4203},
  year={2013}
}

@article{gourmelon,
	Author = {Gourmelon, Nicolas},
	Hal_Id = {hal-00387460},
	Hal_Version = {v1},
	Journal = {{Ergodic Theory and Dynamical Systems}},
	Keywords = {Dominated splitting ; partially hyperbolic ; adapted metric ; Banach bundle ; linear cocycle},
	Number = {6},
	Pages = {1839--1849},
	Publisher = {{Cambridge University Press (CUP)}},
	Title = {{Adapted Metrics for Dominated splittings.}},
	Url = {https://hal.archives-ouvertes.fr/hal-00387460},
	Volume = {27},
	Year = {2007},
	Bdsk-Url-1 = {https://hal.archives-ouvertes.fr/hal-00387460}}

@article{sinai,
	Author = {Ya. G. Sinai},
	Journal = {Izv. Akad. Nauk SSSR Ser. Mat.},
	Title = {Asymptotic behavior of closed geodesics on compact manifolds with negative curvature},
	Year = {1966}}

@article{guillemin1977lectures,
	Author = {Guillemin, Victor},
	Doi = {10.1215/S0012-7094-77-04422-2},
	Fjournal = {Duke Mathematical Journal},
	Journal = {Duke Math. J.},
	Month = {09},
	Number = {3},
	Pages = {485--517},
	Publisher = {Duke University Press},
	Title = {Lectures on spectral theory of elliptic operators},
	Url = {https://doi.org/10.1215/S0012-7094-77-04422-2},
	Volume = {44},
	Year = {1977},
	Bdsk-Url-1 = {https://doi.org/10.1215/S0012-7094-77-04422-2},
	Bdsk-Url-2 = {http://dx.doi.org/10.1215/S0012-7094-77-04422-2}}

@book{hor1,
	Author = {H{\"o}rmander, L.},
	Isbn = {9783540523437},
	Lccn = {89261345},
	Publisher = {Springer-Verlag},
	Series = {Springer Study Edition},
	Title = {The analysis of linear partial differential operators: Distribution theory and Fourier analysis},
	Url = {https://books.google.fr/books?id=UpdaAAAAYAAJ},
	Year = {1990},
	Bdsk-Url-1 = {https://books.google.fr/books?id=UpdaAAAAYAAJ}}

@article{faure2011upper,
	Abstract = {Using a semiclassical approach we show that the spectrum of a smooth Anosov vector field V on a compact manifold is discrete (in suitable anisotropic Sobolev spaces) and then we provide an upper bound for the density of eigenvalues of the operator (‚àíi)V, called Ruelle resonances, close to the real axis and for large real parts.},
	Author = {Faure, Fr{\'e}d{\'e}ric and Sj{\"o}strand, Johannes},
	Day = {13},
	Doi = {10.1007/s00220-011-1349-z},
	Issn = {1432-0916},
	Journal = {Communications in Mathematical Physics},
	Month = {Oct},
	Number = {2},
	Pages = {325},
	Title = {Upper Bound on the Density of Ruelle Resonances for Anosov Flows},
	Url = {https://doi.org/10.1007/s00220-011-1349-z},
	Volume = {308},
	Year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1007/s00220-011-1349-z},
	Bdsk-Url-2 = {http://dx.doi.org/10.1007/s00220-011-1349-z}}


@book{zworski,
  title={Semiclassical Analysis},
  author={Zworski, M.},
  isbn={9780821883204},
  lccn={2012010649},
  series={Graduate studies in mathematics},
  url={https://books.google.fr/books?id=3Z0CAQAAQBAJ},
  year={2012},
  publisher={American Mathematical Society}
}

@book{kato1976perturbation,
      author        = "Kato, Tosio",
      title         = "{Perturbation theory for linear operators; 2nd ed.}",
      publisher     = "Springer",
      address       = "Berlin",
      series        = "Grundlehren Math. Wiss.",
      year          = "1976",
      url           = "https://cds.cern.ch/record/101545",
}

@article{ruelle1976zeta,
  title={Zeta-functions for expanding maps and Anosov flows},
  author={Ruelle, David},
  journal={Inventiones mathematicae},
  volume={34},
  number={3},
  pages={231--242},
  year={1976},
  publisher={Springer}
}


@article{giulietti2013anosov,
  title={Anosov flows and dynamical zeta functions},
  author={Giulietti, Paolo and Liverani, Carlangelo and Pollicott, Mark},
  journal={Annals of Mathematics},
  pages={687--773},
  year={2013},
  publisher={JSTOR}
}


@article{pollicott1985rate,
  title={On the rate of mixing of Axiom A flows},
  author={Pollicott, Mark},
  journal={Inventiones mathematicae},
  volume={81},
  number={3},
  pages={413--426},
  year={1985},
  publisher={Springer}
}

@inproceedings{dyatlov2016pollicott,
  title={Pollicott--Ruelle resonances for open systems},
  author={Dyatlov, Semyon and Guillarmou, Colin},
  booktitle={Annales Henri Poincar{\'e}},
  volume={17},
  number={11},
  pages={3089--3146},
  year={2016},
  organization={Springer}
}

@article{margulis1969applications,
  title={Applications of ergodic theory to the investigation of manifolds of negative curvature},
  author={Margulis, Gregorii A},
  journal={Functional analysis and its applications},
  volume={3},
  number={4},
  pages={335--336},
  year={1969},
  publisher={Springer}
}

@article{anosov1967geodesic,
  title={Geodesic flows on closed Riemannian manifolds of negative curvature},
  author={Anosov, Dmitry Victorovich},
  journal={Trudy Matematicheskogo Instituta Imeni VA Steklova},
  volume={90},
  pages={3--210},
  year={1967},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian Academy of Sciences}
}

@article{parry1983analogue,
  title={An analogue of the prime number theorem for closed orbits of Axiom A flows},
  author={Parry, William and Pollicott, Mark},
  journal={Annals of mathematics},
  pages={573--591},
  year={1983},
  publisher={JSTOR}
}

@article{rugh1996generalized,
  title={Generalized Fredholm determinants and Selberg zeta functions for Axiom A dynamical systems},
  author={Rugh, Hans Henrik},
  journal={Ergodic Theory and Dynamical Systems},
  volume={16},
  number={4},
  pages={805--819},
  year={1996},
  publisher={Cambridge University Press}
}

@article{fried1995meromorphic,
  title={Meromorphic zeta functions for analytic flows},
  author={Fried, David},
  journal={Communications in mathematical physics},
  volume={174},
  number={1},
  pages={161--190},
  year={1995},
  publisher={Springer}
}

@article{dang2016spectral,
  title={Spectral analyss of Morse-Smale gradient flows},
  author={Dang, Nguyen Viet and Riviere, Gabriel},
  journal={arXiv preprint arXiv:1605.05516},
  year={2016}
}

@inproceedings{baladi2007anisotropic,
  title={Anisotropic H{\"o}lder and Sobolev spaces for hyperbolic diffeomorphisms (Espaces anisotropes de types H{\"o}lder et Sobolev)},
  author={Baladi, Viviane and Tsujii, Masato},
  booktitle={Annales de l'institut Fourier},
  volume={57},
  number={1},
  pages={127--154},
  year={2007}
}

@article{blank2002ruelle,
  title={Ruelle--Perron--Frobenius spectrum for Anosov maps},
  author={Blank, Michael and Keller, Gerhard and Liverani, Carlangelo},
  journal={Nonlinearity},
  volume={15},
  number={6},
  pages={1905},
  year={2002},
  publisher={IOP Publishing}
}


@article{gouezel2006banach,
  title={Banach spaces adapted to Anosov systems},
  author={Gou{\"e}zel, S{\'e}bastien and Liverani, Carlangelo},
  journal={Ergodic Theory and dynamical systems},
  volume={26},
  number={1},
  pages={189--217},
  year={2006},
  publisher={Cambridge University Press}
}

@article{liverani2004contact,
  title={On contact Anosov flows},
  author={Liverani, Carlangelo},
  journal={Annals of mathematics},
  pages={1275--1312},
  year={2004},
  publisher={JSTOR}
}

@article{liverani2005fredholm,
  title={Fredholm determinants, Anosov maps and Ruelle resonances},
  author={Liverani, Carlangelo},
  journal={arXiv preprint math/0505049},
  year={2005}
}

@article{butterley2007smooth,
  title={Smooth Anosov flows: correlation spectra and stability},
  author={Butterley, Oliver and Liverani, Carlangelo},
  journal={J. Mod. Dyn},
  volume={1},
  number={2},
  pages={301--322},
  year={2007},
  publisher={Citeseer}
}

@article{smale1967differentiable,
  title={Differentiable dynamical systems},
  author={Smale, Stephen},
  journal={Bulletin of the American mathematical Society},
  volume={73},
  number={6},
  pages={747--817},
  year={1967}
}


@book{gallot2004riemannian,
  title={Riemannian Geometry},
  author={Gallot, S. and Hulin, D. and Lafontaine, J.},
  isbn={9783540204930},
  lccn={90022646},
  series={Universitext},
  url={https://books.google.fr/books?id=6F4Umpws\_gUC},
  year={2004},
  publisher={Springer Berlin Heidelberg}
}

@book{hatcher2002algebraic,
  title={Algebraic Topology},
  author={Hatcher, A.},
  isbn={9780521795401},
  lccn={00065166},
  series={Algebraic Topology},
  url={https://books.google.fr/books?id=BjKs86kosqgC},
  year={2002},
  publisher={Cambridge University Press}
}


@article{smale1967differentiable,
  title={Differentiable dynamical systems},
  author={Smale, Stephen},
  journal={Bulletin of the American mathematical Society},
  volume={73},
  number={6},
  pages={747--817},
  year={1967}
}


@article{dyatlov2017ruelle,
  title={Ruelle zeta function at zero for surfaces},
  author={Dyatlov, Semyon and Zworski, Maciej},
  journal={Inventiones mathematicae},
  volume={210},
  number={1},
  pages={211--229},
  year={2017},
  publisher={Springer}
}

@book{hor3,
  title={The Analysis of Linear Partial Differential Operators III: Pseudo-Differential Operators},
  author={H{\"o}rmander, L.},
  isbn={9783540138280},
  lccn={83000616},
  series={Grundlehren der mathematischen Wissenschaften},
  url={https://books.google.fr/books?id=Bv4KlsyxSsYC},
  year={1994},
  publisher={Springer Berlin Heidelberg}
}

@article{dyatlov2017mathematical,
  title={Mathematical theory of scattering resonances},
  author={Dyatlov, Semyon and Zworski, Maciej},
  journal={book in progress},
  year={2017}
}

@article{selberg1956,
      author        = "Selberg, A",
      title         = "{Harmonic analysis and discontinuous groups in weakly
                       symmetric Riemannian spaces with applications to Dirichlet
                       series}",
      journal       = "J. Indian Math. Soc.",
      volume        = "20",
      pages         = "47-87",
      year          = "1956",
      url           = "http://cds.cern.ch/record/427143",
}

@article{rugh1996generalized,
  title={Generalized Fredholm determinants and Selberg zeta functions for Axiom A dynamical systems},
  author={Rugh, Hans Henrik},
  journal={Ergodic Theory and Dynamical Systems},
  volume={16},
  number={4},
  pages={805--819},
  year={1996},
  publisher={Cambridge University Press}
}

@article{fried1995meromorphic,
  title={Meromorphic zeta functions for analytic flows},
  author={Fried, David},
  journal={Communications in mathematical physics},
  volume={174},
  number={1},
  pages={161--190},
  year={1995},
  publisher={Springer}
}

@book{parry1990zeta,
  title={Zeta Functions and the Periodic Orbit Structure of Hyperbolic Dynamics},
  author={Parry, W. and Pollicott, M.},
  lccn={93194624},
  url={https://books.google.fr/books?id=NQ0ZAQAAIAAJ},
  year={1990},
  publisher={Soci{\'e}t{\'e} math{\'e}matique de France}
}

@article{blank2002ruelle,
  title={Ruelle--Perron--Frobenius spectrum for Anosov maps},
  author={Blank, Michael and Keller, Gerhard and Liverani, Carlangelo},
  journal={Nonlinearity},
  volume={15},
  number={6},
  pages={1905},
  year={2002},
  publisher={IOP Publishing}
}


  	
@article{kitaev99,
  author={A Yu Kitaev},
  title={Fredholm determinants for hyperbolic diffeomorphisms of finite smoothness},
  journal={Nonlinearity},
  volume={12},
  number={1},
  pages={141},
  url={http://stacks.iop.org/0951-7715/12/i=1/a=008},
  year={1999},
  abstract={Given a map ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img1.gif] and a function ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img2.gif] , a `Fredholm determinant' can be defined as a formal power series ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img3.gif] . The coefficients ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img4.gif] are related to the periodic points of ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img5.gif] . Assume that ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img5.gif] is a hyperbolic diffeomorphism of class ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img7.gif] , and ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img8.gif] belongs to ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img9.gif] . Then the Fredholm determinant is analytic in the disc of radius ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img10.gif] , where ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img11.gif] is a hyperbolicity index of ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img5.gif] (roughly speaking, ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img5.gif] is ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img14.gif] -contracting in one direction and ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img15.gif] -expanding in the other direction). In the ##IMG## [http://ej.iop.org/images/0951-7715/12/1/008/img16.gif] case, the Fredholm determinant is an entire function.}
}

@article{dyatlov2018afterword,
  title={Afterword: Dynamical zeta functions for Axiom A flows},
  author={Dyatlov, Semyon and Guillarmou, Colin},
  journal={Bulletin of the American Mathematical Society},
  volume={55},
  number={3},
  pages={337--342},
  year={2018}
}


@article{faure2017semiclassical,
  title={The semiclassical zeta function for geodesic flows on negatively curved manifolds},
  author={Faure, Fr{\'e}d{\'e}ric and Tsujii, Masato},
  journal={Inventiones mathematicae},
  volume={208},
  number={3},
  pages={851--998},
  year={2017},
  publisher={Springer}
}

@article{melrose1994spectral,
  title={Spectral and scattering theory for the Laplacian on asymptotically Euclidian spaces},
  author={Melrose, Richard B},
  year={1994}
}

@article{vasy2013microlocal,
  title={Microlocal analysis of asymptotically hyperbolic and Kerr-de Sitter spaces (with an appendix by Semyon Dyatlov)},
  author={Vasy, Andr{\'a}s},
  journal={Inventiones mathematicae},
  volume={194},
  number={2},
  pages={381--513},
  year={2013},
  publisher={Springer}
}


@article{hadfield2018zeta,
  title={Zeta function at zero for surfaces with boundary},
  author={Hadfield, Charles},
  journal={arXiv preprint arXiv:1803.10982},
  year={2018}
}

@article{guillarmou2018classical,
  title={Classical and quantum resonances for hyperbolic surfaces},
  author={Guillarmou, Colin and Hilgert, Joachim and Weich, Tobias},
  journal={Mathematische Annalen},
  volume={370},
  number={3-4},
  pages={1231--1275},
  year={2018},
  publisher={Springer}
}

@article{patterson2001divisor,
  title={The divisor of Selberg's zeta function for Kleinian groups},
  author={Patterson, Samuel J and Perry, Peter A and others},
  journal={Duke Mathematical Journal},
  volume={106},
  number={2},
  pages={321--390},
  year={2001},
  publisher={Duke University Press}
}


@article{huber1961zur,
  title={Zur analytischen Theorie hyperbolischer Raumformen und Bewegungsgruppen. II},
  author={Huber, Heinz},
  journal={Mathematische Annalen},
  volume={142},
  number={4},
  pages={385--398},
  year={1961},
  publisher={Springer}
}

@article{braverman2007refined,
  title={Refined analytic torsion as an element of the determinant line},
  author={Braverman, Maxim and Kappeler, Thomas},
  journal={Geometry \& Topology},
  volume={11},
  number={1},
  pages={139--213},
  year={2007},
  publisher={Mathematical Sciences Publishers}
}

@article{braverman2008refined,
  title={Refined analytic torsion},
  author={Braverman, Maxim and Kappeler, Thomas and others},
  journal={Journal of Differential Geometry},
  volume={78},
  number={2},
  pages={193--267},
  year={2008},
  publisher={Lehigh University}
}

@article{braverman2007ray,
  title={Ray--Singer type theorem for the refined analytic torsion},
  author={Braverman, Maxim and Kappeler, Thomas},
  journal={Journal of Functional Analysis},
  volume={243},
  number={1},
  pages={232--256},
  year={2007},
  publisher={Elsevier}
}

@article{dang2017topology,
  title={Topology of Pollicott-Ruelle resonant states},
  author={Dang, Nguyen Viet and Riviere, Gabriel},
  journal={arXiv preprint arXiv:1703.08037},
  year={2017}
}

@article{dang2018fried,
  title={Fried conjecture in small dimensions},
  author={Dang, Nguyen Viet and Guillarmou, Colin and Rivi{\`e}re, Gabriel and Shen, Shu},
  year={2018},
  journal={To appear}
}


@article{giulietti2013anosov,
  title={Anosov flows and dynamical zeta functions},
  author={Giulietti, Paolo and Liverani, Carlangelo and Pollicott, Mark},
  journal={Annals of Mathematics},
  pages={687--773},
  year={2013},
  publisher={JSTOR}
}


@book{voisin_2002, place={Cambridge}, series={Cambridge Studies in Advanced Mathematics}, title={Hodge Theory and Complex Algebraic Geometry I}, volume={1}, DOI={10.1017/CBO9780511615344}, publisher={Cambridge University Press}, author={Voisin, Claire}, editor={Schneps, LeilaTranslator}, year={2002}, collection={Cambridge Studies in Advanced Mathematics}}


@article{bonthonneau2018flow,
  title={Flow-independent Anisotropic space, and perturbation of resonances},
  author={Bonthonneau, Yannick Guedes},
  journal={arXiv preprint arXiv:1806.08125},
  year={2018}
}


@article{ray1971r,
  title={R-torsion and the Laplacian on Riemannian manifolds},
  author={Ray, Daniel B and Singer, Isadore M},
  journal={Advances in Mathematics},
  volume={7},
  number={2},
  pages={145--210},
  year={1971},
  publisher={Elsevier}
}


@inproceedings{reidemeister1935homotopieringe,
  title={Homotopieringe und linsenr{\"a}ume},
  author={Reidemeister, Kurt},
  booktitle={Abhandlungen aus dem Mathematischen Seminar der Universit{\"a}t Hamburg},
  volume={11},
  number={1},
  pages={102--109},
  year={1935},
  organization={Springer}
}


@article{atiyah1967lefschetz,
  title={A Lefschetz fixed point formula for elliptic complexes: I},
  author={Atiyah, Michael Francis and Bott, Raoul},
  journal={Annals of Mathematics},
  pages={374--407},
  year={1967},
  publisher={JSTOR}
}


@article{franz1935torsion,
  title={{\"U}ber die Torsion einer {\"U}berdeckung.},
  author={Franz, Wolfgang},
  journal={Journal f{\"u}r die reine und angewandte Mathematik},
  volume={173},
  pages={245--254},
  year={1935}
}


@article{cheeger1979analytic,
  title={Analytic torsion and the heat equation},
  author={Cheeger, Jeff},
  journal={Annals of Mathematics},
  volume={109},
  number={2},
  pages={259--321},
  year={1979},
  publisher={JSTOR}
}

@article{muller1978analytic,
  title={Analytic torsion and R-torsion of Riemannian manifolds},
  author={M{\"u}ller, Werner},
  journal={Advances in Mathematics},
  volume={28},
  number={3},
  pages={233--305},
  year={1978},
  publisher={Academic Press}
}

@article{muller1993analytic,
  title={Analytic torsion and R-torsion for unimodular representations},
  author={Muller, Werner},
  journal={Journal of the American Mathematical Society},
  volume={6},
  number={3},
  pages={721--753},
  year={1993},
  publisher={JSTOR}
}

@article{bismut1992extension,
  title={An extension of a theorem by Cheeger and M{\"u}ller},
  author={Bismut, Jean-Michel and Zhang, Weiping},
  journal={Ast{\'e}risque},
  volume={205},
  pages={235},
  year={1992}
}

@incollection {fried1987lefschetz,
    AUTHOR = {Fried, David},
     TITLE = {Lefschetz formulas for flows},
 BOOKTITLE = {The {L}efschetz centennial conference, {P}art {III} ({M}exico
              {C}ity, 1984)},
    SERIES = {Contemp. Math.},
    VOLUME = {58},
     PAGES = {19--69},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1987},
   MRCLASS = {58F25 (58F22)},
  MRNUMBER = {893856},
MRREVIEWER = {S. Yu. Pilyugin},
}

@inproceedings{fried1986zeta,
  title={The zeta functions of Ruelle and Selberg. I},
  author={Fried, David},
  booktitle={Annales scientifiques de l'Ecole normale sup{\'e}rieure},
  volume={19},
  number={4},
  pages={491--517},
  year={1986}
}

@article{ruelle1976zeta,
  title={Zeta-functions for expanding maps and Anosov flows},
  author={Ruelle, David},
  journal={Inventiones mathematicae},
  volume={34},
  number={3},
  pages={231--242},
  year={1976},
  publisher={Springer}
}

@article{fried1986analytic,
  title={Analytic torsion and closed geodesics on hyperbolic manifolds},
  author={Fried, David},
  journal={Inventiones mathematicae},
  volume={84},
  number={3},
  pages={523--540},
  year={1986},
  publisher={Springer}
}

@article{fried1983homological,
  title={Homological identities for closed orbits},
  author={Fried, David},
  journal={Inventiones Mathematicae},
  volume={71},
  number={2},
  pages={419--442},
  year={1983},
  publisher={Springer}
}

@article{fried1995meromorphic,
  title={Meromorphic zeta functions for analytic flows},
  author={Fried, David},
  journal={Communications in mathematical physics},
  volume={174},
  number={1},
  pages={161--190},
  year={1995},
  publisher={Springer}
}

@article{moscovici1991r,
  title={R-torsion and zeta functions for locally symmetric manifolds},
  author={Moscovici, Henri and Stanton, Robert J},
  journal={Inventiones mathematicae},
  volume={105},
  number={1},
  pages={185--216},
  year={1991},
  publisher={Springer}
}

@article{shen2017analytic,
  title={Analytic torsion, dynamical zeta functions, and the Fried conjecture},
  author={Shen, Shu},
  journal={Analysis \& PDE},
  volume={11},
  number={1},
  pages={1--74},
  year={2017},
  publisher={Mathematical Sciences Publishers}
}

@article{zworski2018commentary,
  title={Commentary on \D2Differentiable dynamical systems\D3 by Stephen Smale},
  author={Zworski, Maciej},
  journal={Bulletin of the American Mathematical Society},
  volume={55},
  number={3},
  pages={331--336},
  year={2018}
}


@article{turaev1986reidemeister,
  title={Reidemeister torsion in knot theory},
  author={Turaev, Vladimir G},
  journal={Russian Mathematical Surveys},
  volume={41},
  number={1},
  pages={119},
  year={1986},
  publisher={IOP Publishing}
}

@article{turaev1990euler,
  title={Euler structures, nonsingular vector fields, and torsions of Reidemeister type},
  author={Turaev, Vladimir Georgievich},
  journal={Mathematics of the USSR-Izvestiya},
  volume={34},
  number={3},
  pages={627},
  year={1990},
  publisher={IOP Publishing}
}

@article {farber2000poincare,
    AUTHOR = {Farber, Michael and Turaev, Vladimir},
     TITLE = {Poincar\'{e}-{R}eidemeister metric, {E}uler structures, and
              torsion},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {520},
      YEAR = {2000},
     PAGES = {195--225},
      ISSN = {0075-4102},
   MRCLASS = {58J52 (57R20)},
  MRNUMBER = {1748274},
MRREVIEWER = {Yi-Jen Lee},
       DOI = {10.1515/crll.2000.021},
       URL = {https://doi.org/10.1515/crll.2000.021},
}

@article{turaev1997torsion,
  title={Torsion invariants of $ Spin^c $-structures on 3-manifolds},
  author={Turaev, Vladimir},
  journal={Mathematical Research Letters},
  volume={4},
  number={5},
  pages={679--695},
  year={1997},
  publisher={International Press of Boston}
}


@article{burghelea2006euler,
  title={Euler structures, the variety of representations and the Milnor--Turaev torsion},
  author={Burghelea, Dan and Haller, Stefan},
  journal={Geometry \& Topology},
  volume={10},
  number={2},
  pages={1185--1238},
  year={2006},
  publisher={Mathematical Sciences Publishers}
}

@article{burghelea2007complex,
  title={Complex-valued Ray--Singer torsion},
  author={Burghelea, Dan and Haller, Stefan},
  journal={Journal of Functional Analysis},
  volume={248},
  number={1},
  pages={27--78},
  year={2007},
  publisher={Elsevier}
}

@incollection{burghelea2008torsion,
  title={Torsion, as a function on the space of representations},
  author={Burghelea, Dan and Haller, Stefan},
  booktitle={C*-algebras and Elliptic Theory II},
  pages={41--66},
  year={2008},
  publisher={Springer}
}


@article{moscovici1991r,
  title={R-torsion and zeta functions for locally symmetric manifolds},
  author={Moscovici, Henri and Stanton, Robert J},
  journal={Inventiones mathematicae},
  volume={105},
  number={1},
  pages={185--216},
  year={1991},
  publisher={Springer}
}

@article{shen2017analytic,
  title={Analytic torsion, dynamical zeta functions, and the Fried conjecture},
  author={Shen, Shu},
  journal={Analysis \& PDE},
  volume={11},
  number={1},
  pages={1--74},
  year={2017},
  publisher={Mathematical Sciences Publishers}
}


@article{sanchez1993lefschetz,
  title={Lefschetz formulae for Anosov flows on 3-manifolds},
  author={S{\'a}nchez-Morgado, H{\'e}ctor},
  journal={Ergodic Theory and Dynamical Systems},
  volume={13},
  number={2},
  pages={335--347},
  year={1993},
  publisher={Cambridge University Press}
}

@article{sanchez1996r,
  title={R-torsion and zeta functions for analytic Anosov flows on 3-manifolds},
  author={S{\'a}nchez-Morgado, H{\'e}ctor},
  journal={Transactions of the American Mathematical Society},
  volume={348},
  number={3},
  pages={963--973},
  year={1996}
}

@incollection {baladi2005anisotropic,
    AUTHOR = {Baladi, Viviane},
     TITLE = {Anisotropic {S}obolev spaces and dynamical transfer operators:
              {$C^\infty$} foliations},
 BOOKTITLE = {Algebraic and topological dynamics},
    SERIES = {Contemp. Math.},
    VOLUME = {385},
     PAGES = {123--135},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {2005},
   MRCLASS = {37D20 (37A25 37C30 46E35)},
  MRNUMBER = {2180233},
MRREVIEWER = {Masato Tsujii},
       DOI = {10.1090/conm/385/07194},
       URL = {https://doi.org/10.1090/conm/385/07194},
}


@article{butterley2013robustly,
  title={Robustly invariant sets in fiber contracting bundle flows},
  author={Butterley, Oliver and Liverani, Carlangelo},
  journal={Journal of Modern Dynamics},
  volume={7},
  number={2},
  pages={255--267},
  year={2013},
  publisher={Univerza v Novi Gorici}
}


@article{hutchings1999reidemeister,
  title={Reidemeister torsion in generalized Morse theory},
  author={Hutchings, Michael},
  journal={arXiv preprint math/9907066},
  year={1999}
}


@article{hutchings1999circle1,
  title={Circle-valued Morse theory, Reidemeister torsion, and Seiberg--Witten invariants of 3-manifolds},
  author={Hutchings, Michael and Lee, Yi-Jen},
  journal={Topology},
  volume={38},
  number={4},
  pages={861--888},
  year={1999},
  publisher={Elsevier}
}

@article{hutchings1999circle,
  title={Circle-valued Morse theory and Reidemeister torsion},
  author={Hutchings, Michael and Lee, Yi-Jen},
  journal={Geometry \& Topology},
  volume={3},
  number={1},
  pages={369--396},
  year={1999},
  publisher={Mathematical Sciences Publishers}
}

@inproceedings{braverman2007comparison,
  title={Comparison of the refined analytic and the Burghelea-Haller torsions},
  author={Braverman, Maxim and Kappeler, Thomas},
  booktitle={Annales de l'institut Fourier},
  volume={57},
  number={7},
  pages={2361--2387},
  year={2007}
}


@book {turaev2001introduction,
    AUTHOR = {Turaev, Vladimir},
     TITLE = {Introduction to combinatorial torsions},
    SERIES = {Lectures in Mathematics ETH Z\"{u}rich},
      NOTE = {Notes taken by Felix Schlenk},
 PUBLISHER = {Birkh\"{a}user Verlag, Basel},
      YEAR = {2001},
     PAGES = {viii+123},
      ISBN = {3-7643-6403-3},
   MRCLASS = {57Q10 (19J10 57M27)},
  MRNUMBER = {1809561},
MRREVIEWER = {Joan Porti},
       DOI = {10.1007/978-3-0348-8321-4},
       URL = {https://doi.org/10.1007/978-3-0348-8321-4},
}

			
@book {steenrod1999the,
    AUTHOR = {Steenrod, Norman},
     TITLE = {The topology of fibre bundles},
    SERIES = {Princeton Landmarks in Mathematics},
      NOTE = {Reprint of the 1957 edition,
              Princeton Paperbacks},
 PUBLISHER = {Princeton University Press, Princeton, NJ},
      YEAR = {1999},
     PAGES = {viii+229},
      ISBN = {0-691-00548-6},
   MRCLASS = {55-02 (01A75 55Rxx)},
  MRNUMBER = {1688579},
}

@article{braverman2017refined,
  title={Refined analytic torsion as analytic function on the representation variety and applications},
  author={Braverman, Maxim and Vertman, Boris},
  journal={Annales math{\'e}matiques du Qu{\'e}bec},
  volume={41},
  number={1},
  pages={67--96},
  year={2017},
  publisher={Springer}
}


@article{bonthonneau2018flow,
  title={Flow-independent Anisotropic space, and perturbation of resonances},
  author={Bonthonneau, Yannick Guedes},
  journal={arXiv preprint arXiv:1806.08125},
  year={2018}
}


@article{de1936nouveaux,
  title={Sur les nouveaux invariants topologiques de M. Reidemeister},
  author={de Rham, G},
  journal={\foreignlanguage{russian}{?????. ??}},
  volume={1},
  number={43},
  pages={5},
  year={1936}
}


@article{burghelea2008dynamics,
  title={Dynamics, Laplace transform and spectral geometry},
  author={Burghelea, Dan and Haller, Stefan},
  journal={Journal of Topology},
  volume={1},
  number={1},
  pages={115--151},
  year={2008},
  publisher={Wiley Online Library}
}


@book{baladi2018dynamical,
  title={Dynamical zeta functions and dynamical determinants for hyperbolic maps},
  author={Baladi, Viviane},
  year={2018},
  publisher={Springer}
}

@book{audin2014morse,
  title={Morse theory and Floer homology},
  author={Audin, Mich{\`e}le and Damian, Mihai},
  publisher={Springer}
}

@book{nicolaescu2003reidemeister,
  title={The Reidemeister Torsion of 3-manifolds},
  author={Nicolaescu, L.I.},
  isbn={9783110173833},
  lccn={2002041469},
  series={De Gruyter studies in mathematics},
  url={https://books.google.com.sg/books?id=qZRGjI66dhIC},
  year={2003},
  publisher={Walter de Gruyter}
}



@book{dyatlov2019mathematical,
  title={Mathematical Theory of Scattering Resonances},
  author={Dyatlov, S. and Zworski, M.},
  isbn={9781470443665},
  lccn={2019006281},
  series={Graduate Studies in Mathematics},
  url={https://books.google.fr/books?id=QtqSwwEACAAJ},
  year={2019},
  publisher={American Mathematical Society}
}


@article{huang2007refined,
  title={Refined analytic torsion: comparison theorems and examples},
  author={Huang, Rung-Tzung and others},
  journal={Illinois Journal of Mathematics},
  volume={51},
  number={4},
  pages={1309--1327},
  year={2007},
  publisher={University of Illinois at Urbana-Champaign}
}


@article{harvey2001finite,
  title={Finite volume flows and Morse theory},
  author={Harvey, F Reese and Lawson Jr, H Blaine},
  journal={Annals of Mathematics},
  volume={153},
  number={1},
  pages={1--25},
  year={2001},
  publisher={PRINCETON UNIVERSITY}
}

@article{faure2008semi,
  title={Semi-classical approach for Anosov diffeomorphisms and Ruelle resonances},
  author={Faure, Fr{\'e}d{\'e}ric and Roy, Nicolas and Sj{\"o}strand, Johannes},
  journal={arXiv preprint arXiv:0802.1780},
  year={2008}
}


@article{turaev1986reidemeister,
  title={Reidemeister torsion in knot theory},
  author={Turaev, Vladimir G},
  journal={Russian Mathematical Surveys},
  volume={41},
  number={1},
  pages={119},
  year={1986},
  publisher={IOP Publishing}
}




@article{hassannezhad2016eigenvalue,
  title={Eigenvalue inequalities on Riemannian manifolds with a lower Ricci curvature bound},
  author={Hassannezhad, Asma and Kokarev, Gerasim and Polterovich, Iosif},
  journal={Journal of Spectral Theory},
  volume={6},
  number={4},
  pages={807--835},
  year={2016}
}

@article{deitmar2019benjamini,
  title={Benjamini--Schramm and spectral convergence},
  author={Deitmar, Anton},
  journal={L‚ÄôEnseignement Math{\'e}matique},
  volume={64},
  number={3},
  pages={371--394},
  year={2019}
}




@book{deitmar2014principles,
  title={Principles of harmonic analysis},
  author={Deitmar, Anton and Echterhoff, Siegfried},
  year={2014},
  publisher={Springer}
}


@article{lenz2014ihara,
  title={The Ihara Zeta function for infinite graphs},
  author={Lenz, Daniel and Pogorzelski, Felix and Schmidt, Marcel},
  journal={arXiv preprint arXiv:1408.3522},
  year={2014}
}

@article{dang2020poincar,
  title={Poincar\'e series and linking of Legendrian knots},
  author={Dang, Nguyen Viet and Rivi{\`e}re, Gabriel},
  journal={arXiv preprint arXiv:2005.13235},
  year={2020}
}

@book {klingenberg2011riemannian,
      author = "Wilhelm P.A. Klingenberg",
      title = "Riemannian Geometry",
      year = "03 May. 2011",
      publisher = "De Gruyter",
      address = "Berlin, Boston",
      isbn = "978-3-11-090512-0",
      doi = "https://doi.org/10.1515/9783110905120",
      url = "https://www.degruyter.com/view/title/3533"
}

@article{klingenberg1974riemannian,
  title={Riemannian manifolds with geodesic flow of Anosov type},
  author={Klingenberg, Wilhelm},
  journal={Annals of Mathematics},
  pages={1--13},
  year={1974},
  publisher={JSTOR}
}


@book {singer1976lecture,
      author = "I. M. Singer and J. A. Thorpe",
      title = "Lecture Notes on Elementary Topology and Geometry",
      year = "1976",
      publisher = "Springer Verlag",
      address = "Berlin, Boston",
      isbn = "0-387-90202-3",
      doi = "",
      url = ""
}



@inproceedings{delange1954generalisation,
  title={G{\'e}n{\'e}ralisation du th{\'e}oreme de Ikehara},
  author={Delange, Hubert},
  booktitle={Annales scientifiques de l'{\'E}cole Normale Sup{\'e}rieure},
  volume={71},
  number={3},
  pages={213--242},
  year={1954}
}



@article{kato2014remark,
  title={A remark on the Wiener-Ikehara Tauberian theorem},
  author={Kato, Ryo},
  journal={arXiv preprint arXiv:1406.0427},
  year={2014}
}



@article{wiener1932tauberian,
  title={Tauberian theorems},
  author={Wiener, Norbert},
  journal={Annals of mathematics},
  pages={1--100},
  year={1932},
  publisher={JSTOR}
}

@inproceedings{Jost1997NonpositiveCG,
  title={Nonpositive Curvature: Geometric And Analytic Aspects},
  author={J. Jost},
  year={1997}
}

@article{margulis1969applications,
  title={Applications of ergodic theory to the investigation of manifolds of negative curvature},
  author={Margulis, Grigorii Aleksandrovich},
  journal={Funktsional'nyi Analiz i ego Prilozheniya},
  volume={3},
  number={4},
  pages={89--90},
  year={1969},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}



@inproceedings{anantharaman2000precise,
  title={Precise counting results for closed orbits of Anosov flows},
  author={Anantharaman, Nalini},
  booktitle={Annales Scientifiques de l’{\'E}cole Normale Sup{\'e}rieure},
  volume={33},
  number={1},
  pages={33--56},
  year={2000},
  organization={Elsevier}
}


@article{phillips1987geodesics,
  title={Geodesics in homology classes},
  author={Phillips, Ralph and Sarnak, Peter},
  journal={Duke Mathematical Journal},
  volume={55},
  number={2},
  pages={287--297},
  year={1987},
  publisher={Duke University Press}
}

@book{lalley1988closed,
  title={Closed geodesics in homology classes on surfaces of variable negative curvature},
  author={Lalley, Steven P.},
  year={1988}
}

@article{pollicott1991homology,
  title={Homology and closed geodesics in a compact negatively curved surface},
  author={Pollicott, Mark},
  journal={American Journal of Mathematics},
  volume={113},
  number={3},
  pages={379--385},
  year={1991},
  publisher={JSTOR}
}


@article{katsuda1988homology,
  title={Homology and closed geodesics in a compact Riemann surface},
  author={Katsuda, Atsushi and Sunada, Toshikazu},
  journal={American Journal of Mathematics},
  volume={110},
  number={1},
  pages={145--155},
  year={1988},
  publisher={JSTOR}
}


@article{parry1983analogue,
  title={An analogue of the prime number theorem for closed orbits of Axiom A flows},
  author={Parry, William and Pollicott, Mark},
  journal={Annals of mathematics},
  pages={573--591},
  year={1983},
  publisher={JSTOR}
}

@article{bowen1972equidistribution,
  title={The equidistribution of closed geodesics},
  author={Bowen, Rufus},
  journal={American Journal of Mathematics},
  volume={94},
  number={2},
  pages={413--423},
  year={1972},
  publisher={JSTOR}
}


@article{bowen1973symbolic,
  title={Symbolic dynamics for hyperbolic flows},
  author={Bowen, Rufus},
  journal={American journal of mathematics},
  volume={95},
  number={2},
  pages={429--460},
  year={1973},
  publisher={JSTOR}
}

@article{paulin2012equilibrium,
  title={Equilibrium states in negative curvature},
  author={Paulin, Fr{\'e}d{\'e}ric and Pollicott, Mark and Schapira, Barbara},
  journal={arXiv preprint arXiv:1211.6242},
  year={2012}
}




@book{sarnak1980prime,
  title = {Prime geodesic theorems},
  author = {Sarnak, Peter},
  publisher = {Stanford University, California},
   year = {1980}
}


@article{lalley1989renewal,
  title={Renewal theorems in symbolic dynamics, with applications to geodesic flows, noneuclidean tessellations and their fractal limits},
  author={Lalley, Steven P},
  journal={Acta mathematica},
  volume={163},
  number={1},
  pages={1--55},
  year={1989},
  publisher={Springer}
}

@article{guillope1986distribution,
  title={Sur la distribution des longueurs des g{\'e}od{\'e}siques ferm{\'e}es d’une surface compacte {\`a} bord totalement g{\'e}od{\'e}sique},
  author={Guillop{\'e}, Laurent},
  journal={Duke Mathematical Journal},
  volume={53},
  number={3},
  pages={827--848},
  year={1986},
  publisher={Duke University Press}
}

@article{mirzakhani2008growth,
  title={Growth of the number of simple closed geodesies on hyperbolic surfaces},
  author={Mirzakhani, Maryam},
  journal={Annals of Mathematics},
  volume={168},
  number={1},
  pages={97--125},
  year={2008},
  publisher={JSTOR}
}


@article{mirzakhani2016counting,
  title={Counting mapping class group orbits on hyperbolic surfaces},
  author={Mirzakhani, Maryam},
  journal={arXiv preprint arXiv:1601.03342},
  year={2016}
}


@article{erlandsson2016counting,
  title={Counting curves in hyperbolic surfaces},
  author={Erlandsson, Viveka and Souto, Juan},
  journal={Geometric and Functional Analysis},
  volume={26},
  number={3},
  pages={729--777},
  year={2016},
  publisher={Springer}
}

@article{pollicott1985asymptotic,
  title={Asymptotic distribution of closed geodesics},
  author={Pollicott, Mark},
  journal={Israel Journal of Mathematics},
  volume={52},
  number={3},
  pages={209--224},
  year={1985},
  publisher={Springer}
}


@article{lyndon1962equation,
  title={The equation $ a^{M}= b^{N}c^{P}$ in a free group.},
  author={Lyndon, Roger C and Sch{\"u}tzenberger, Marcel-Paul},
  journal={Michigan Mathematical Journal},
  volume={9},
  number={4},
  pages={289--298},
  year={1962},
  publisher={The University of Michigan}
}



@article{bonahon1988geometry,
  title={The geometry of Teichm{\"u}ller space via geodesic currents},
  author={Bonahon, Francis},
  journal={Inventiones mathematicae},
  volume={92},
  number={1},
  pages={139--162},
  year={1988},
  publisher={Springer}
}


@article{kifer1994large,
  title={Large deviations, averaging and periodic orbits of dynamical systems},
  author={Kifer, Yuri},
  journal={Communications in mathematical physics},
  volume={162},
  number={1},
  pages={33--46},
  year={1994},
  publisher={Springer}
}



@article{bonahon1986bouts,
  title={Bouts des vari{\'e}t{\'e}s hyperboliques de dimension 3},
  author={Bonahon, Francis},
  journal={Annals of Mathematics},
  volume={124},
  number={1},
  pages={71--158},
  year={1986},
  publisher={JSTOR}
}


@article{otal1990spectre,
  title={Le spectre marqu{\'e} des longueurs des surfaces {\`a} courbure n{\'e}gative},
  author={Otal, Jean-Pierre},
  journal={Annals of Mathematics},
  volume={131},
  number={1},
  pages={151--162},
  year={1990},
  publisher={JSTOR}
}



@article{lalley1996self,
  title={Self-intersections of closed geodesics on a negatively curved surface: statistical regularities},
  author={Lalley, Steven P},
  journal={Convergence in ergodic theory and probability (Columbus, OH, 1993)},
  volume={5},
  pages={263--272},
  year={1996}
}


@article{pugh1983c1,
  title={The C1 closing lemma, including Hamiltonians},
  author={Pugh, Charles C and Robinson, Clark},
  journal={Ergodic Theory and Dynamical Systems},
  volume={3},
  number={2},
  pages={261--313},
  year={1983},
  publisher={Cambridge University Press}
}


@incollection{klingenberg20113,
  title={3.7 The Theorem of the Three Closed Geodesics},
  author={Klingenberg, Wilhelm PA},
  booktitle={Riemannian Geometry},
  pages={337--350},
  year={2011},
  publisher={De Gruyter}
}



@article{tauimanov1993existence,
  title={On the existence of three nonselfintersecting closed geodesics on manifolds homeomorphic to the 2-sphere},
  author={Ta{\u\i}}manov, IA},
  journal={Izvestiya: Mathematics},
  volume={40},
  number={3},
  pages={565},
  year={1993},
  publisher={IOP Publishing}
}

@article{lyusternik1929probleme,
title={Sur le probl\`eme de trois g\'eod\'esiques ferm\'ees sur les surfaces de genre 0},
author={Lyusternik, L. and Schnirelman, L.}
journal={C.R. Acad. Sci. Paris},
volume={189},
date={1929},
pages={269--271}
}

@article{birkhoff1917dynamical,
  title={Dynamical systems with two degrees of freedom},
  author={Birkhoff, George D},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={3},
  number={4},
  pages={314},
  year={1917},
  publisher={National Academy of Sciences}
}


@article{pollicott2006angular,
  title={Angular self-intersections for closed geodesics on surfaces},
  author={Pollicott, Mark and Sharp, Richard},
  journal={Proceedings of the American Mathematical Society},
  volume={134},
  number={2},
  pages={419--426},
  year={2006}
}


@article{roblin2003ergodicite,
  title={Ergodicit{\'e} et {\'e}quidistribution en courbure n{\'e}gative},
  author={Roblin, Thomas},
  journal={M{\'e}moire de la Soci{\'e}t{\'e} math{\'e}matique de France},
  number={95},
  pages={A--96},
  year={2003}
}



@article{guillarmou2017lens,
  title={Lens rigidity for manifolds with hyperbolic trapped sets},
  author={Guillarmou, Colin},
  journal={Journal of the American Mathematical Society},
  volume={30},
  number={2},
  pages={561--599},
  year={2017}
}


@book{Berger_2003,
	doi = {10.1007/978-3-642-18245-7},
	url = {https://doi.org/10.1007/978-3-642-18245-7},
	year = 2003,
	publisher = {Springer Berlin Heidelberg},
	author = {Marcel Berger},
	title = {A Panoramic View of Riemannian Geometry}
}


@article{atiyah1967lefschetz,
  title={A Lefschetz fixed point formula for elliptic complexes: I},
  author={Atiyah, Michael Francis and Bott, Raoul},
  journal={Annals of Mathematics},
  pages={374--407},
  year={1967},
  publisher={JSTOR}
}




@book{bridson2013metric,
  title={Metric spaces of non-positive curvature},
  author={Bridson, Martin R and Haefliger, Andr{\'e}},
  volume={319},
  year={2013},
  publisher={Springer Science \& Business Media}
}


@phdthesis{bonthonneau2015resonances,
  title={R{\'e}sonances du laplacien sur les vari{\'e}t{\'e}s {\`a} pointes},
  author={Bonthonneau, Yannick},
  year={2015},
  school={Universit{\'e} Paris Sud-Paris XI}
}


